Quarkonium Spectroscopy: Beyond One-Gluon Exchange

In this work an improved potential model for quarkonium spectra (charmonium, bottomonium) is constructed. Beside the one-gluon exchange and a linear confinement potential, the model includes systematically effects from two-gluon exchange and the induced interaction (i.e. t-channel exchanges of quark-antiquark bound states). These turn out to be important in order to reproduce correctly the fine- and hyperfine structure of the charmonium and bottomonium states. It is demonstrated that such a satisfactory description of the quarkonium spectra can be obtained with parameters (quark masses, strong coupling constant and string tension) consistent with values of lattice simulations and QCD determinations.

==> 0-Titlepage/titlepage-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Title Page                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\titleheight}
\setlength{\titleheight}{120pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Title Page                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}
\begin{center}
\begin{minipage}{.84\textwidth}
\begin{center}

\vspace{1.\titleheight}


{\bf \huge \centering 
\rule{\textwidth}{1.5pt}

% Draft of the Diploma Thesis
Title
%\\[-9pt]
% \rule{.55\textwidth}{1pt}\\[0pt]


\rule{\textwidth}{1.5pt}}

\vspace{1\titleheight}

{\Large 
Diploma Thesis
}

\vspace{4pt}

{\large
by
}

\vspace{7pt}
 
{\Large 
Johannes Eiglsperger
}

\vspace{.5\titleheight}


{\Large 
January, 2007
}

\vspace{.6\titleheight}

\rule{\textwidth}{1pt}

\vspace{3pt}

%\settowidth{}{×}
\newlength{\tumwidth}
\newlength{\restwidth}
\settowidth{\tumwidth}{{\Large Technische Universit\"at M\"unchen}}
\setlength{\restwidth}{0pt}
\addtolength{\restwidth}{\textwidth}
\addtolength{\restwidth}{-\tumwidth}

\parbox{.48\restwidth}{\centering \oTUM{.17\textwidth}}
\parbox{\tumwidth}{
\Large \centering \vspace{2pt}
Technische Universit\"at M\"unchen

\smallskip

Physik-Departement

\smallskip

T39 (Prof.~Dr.~Wolfram Weise)
}
\parbox{.48\restwidth}{\centering \includegraphics[width=.4\restwidth]{./0-Titlepage/pictures/department-logo-black.eps}}

\vspace{3pt}

\rule{\textwidth}{1pt}

\end{center}
\end{minipage}
% \maketitle
\end{center}
\end{titlepage}

% 
% 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %   Dedication Page                                                           %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\thispagestyle{empty}
% \newenvironment{dedication}
% {\cleardoublepage \thispagestyle{empty} \vspace*{\stretch{1}} \begin{center} \em}
% {\end{center} \vspace*{\stretch{3}} \clearpage}
% \begin{dedication}
% Your dedication goes here \dots
% \end{dedication}
% % \cleardoublepage generates one blank page for the next 'Abstract'
% % to be on an odd page.
% \thispagestyle{empty} \cleardoublepage 
% 
% 


==> 7-Fogtpp-induced/7-Intro.tex <==
In this chapter the improved models discussed in Chapters \ref{Chapt:CpL-induced} \& \ref{Chapt:Fogtpp} are combined into a new model. The chapter is dedicated to a discussion of this model. In the last section the radius-mass relation of bound states is investigated.
